Lower bound on Wyner's Common Information

An important notion of common information between two random variables is due to Wyner. In this paper, we derive a lower bound on Wyner's common information for continuous random variables. The new bound improves on the only other general lower bound on Wyner's common information, which is the mutual information. We also show that the new lower bound is tight for the so-called "Gaussian channels" case, namely, when the joint distribution of the random variables can be written as the sum of a single underlying random variable and Gaussian noises. We motivate this work from the recent variations of Wyner's common information and applications to network data compression problems such as the Gray-Wyner network.

==> defns.tex <==
%%
%% Common definitions
%% Only contains the definitions, not formatting information
%%

%%\usepackage{xspace}
%%\usepackage{mathrsfs}
%% \usepackage{bm}

\let\oldbrace\{
\def\{{\oldbrace\kern0.5pt}

%% A few operator definitions
\def\tr{\mathop{\rm tr}\nolimits}%
\def\var{\mathop{\rm Var}\nolimits}%
\def\Var{\mathop{\rm Var}\nolimits}%
\def\cov{\mathop{\rm Cov}\nolimits}%
\def\Cov{\mathop{\rm Cov}\nolimits}%
\def\diag{\mathop{\rm diag}\nolimits}%
\def\Re{\mathop{\rm Re}\nolimits}%
\def\Im{\mathop{\rm Im}\nolimits}%
\def\rank{\mathop{\rm rank}\nolimits}%
\def\essinf{\mathop{\rm ess\,inf}}%
\def\sgn{\mathop{\rm sgn}\nolimits}%
\def\erfc{\mathop{\rm erfc}\nolimits}%
\newcommand{\supp}{\mathop{\mathrm{supp}}}%

%% General
\newcommand{\nn}{\nonumber}

%% Field 
\newcommand{\q}{\mathsf{q}}
\newcommand{\Fq}{\Field_\q}

%% Mathcal (discrete sets)
\newcommand{\Ac}{\mathcal{A}}
\newcommand{\Bc}{\mathcal{B}}
\newcommand{\Cc}{\mathcal{C}}
\newcommand{\cc}{\text{\footnotesize $\mathcal{C}$} }
\newcommand{\Dc}{\mathcal{D}}
\newcommand{\Ec}{\mathcal{E}}
\newcommand{\Fc}{\mathcal{F}}
\newcommand{\Gc}{\mathcal{G}}
\newcommand{\Hc}{\mathcal{H}}
\newcommand{\Ic}{\mathcal{I}}
\newcommand{\Jc}{\mathcal{J}}
\newcommand{\Kc}{\mathcal{K}}
\newcommand{\Lc}{\mathcal{L}}
\newcommand{\Mc}{\mathcal{M}}
\newcommand{\Nc}{\mathcal{N}}
\newcommand{\Oc}{\mathcal{O}}
\newcommand{\Pc}{\mathcal{P}}
\newcommand{\Qc}{\mathcal{Q}}
\newcommand{\Rc}{\mathcal{R}}
\newcommand{\Sc}{\mathcal{S}}
\newcommand{\Tc}{\mathcal{T}}
\newcommand{\Uc}{\mathcal{U}}
\newcommand{\Vc}{\mathcal{V}}
\newcommand{\Wc}{\mathcal{W}}
\newcommand{\Xc}{\mathcal{X}}
\newcommand{\Yc}{\mathcal{Y}}
\newcommand{\Zc}{\mathcal{Z}}
\newcommand{\Acal}{\mathcal{A}}
\newcommand{\Bcal}{\mathcal{B}}
\newcommand{\Ccal}{\mathcal{C}}
\newcommand{\Dcal}{\mathcal{D}}
\newcommand{\Ecal}{\mathcal{E}}
\newcommand{\Fcal}{\mathcal{F}}
\newcommand{\Gcal}{\mathcal{G}}
\newcommand{\Hcal}{\mathcal{H}}
\newcommand{\Kcal}{\mathcal{K}}
\newcommand{\Ncal}{\mathcal{N}}
\newcommand{\Pcal}{\mathcal{P}}
\newcommand{\Qcal}{\mathcal{Q}}
\newcommand{\Rcal}{\mathcal{R}}
\newcommand{\Scal}{\mathcal{S}}
\newcommand{\Tcal}{\mathcal{T}}
\newcommand{\Ucal}{\mathcal{U}}
\newcommand{\Vcal}{\mathcal{V}}
\newcommand{\Wcal}{\mathcal{W}}
\newcommand{\Xcal}{\mathcal{X}}
\newcommand{\Ycal}{\mathcal{Y}}
\newcommand{\Zcal}{\mathcal{Z}}

%% Mathcal bold (random discrete sets)
\newcommand{\Acb}{\boldsymbol{\mathcal{A}}}
\newcommand{\Bcb}{\boldsymbol{\mathcal{B}}}
\newcommand{\Ccb}{\boldsymbol{\mathcal{C}}}
\newcommand{\Dcb}{\boldsymbol{\mathcal{D}}}
\newcommand{\Ecb}{\boldsymbol{\mathcal{E}}}
\newcommand{\Fcb}{\boldsymbol{\mathcal{F}}}
\newcommand{\Gcb}{\boldsymbol{\mathcal{G}}}
\newcommand{\Hcb}{\boldsymbol{\mathcal{H}}}
\newcommand{\Jcb}{\boldsymbol{\mathcal{J}}}
\newcommand{\Kcb}{\boldsymbol{\mathcal{K}}}
\newcommand{\Ncb}{\boldsymbol{\mathcal{N}}}
\newcommand{\Pcb}{\boldsymbol{\mathcal{P}}}
\newcommand{\Qcb}{\boldsymbol{\mathcal{Q}}}
\newcommand{\Rcb}{\boldsymbol{\mathcal{R}}}
\newcommand{\Scb}{\boldsymbol{\mathcal{S}}}
\newcommand{\Tcb}{\boldsymbol{\mathcal{T}}}
\newcommand{\Ucb}{\boldsymbol{\mathcal{U}}}
\newcommand{\Vcb}{\boldsymbol{\mathcal{V}}}
\newcommand{\Wcb}{\boldsymbol{\mathcal{W}}}
\newcommand{\Xcb}{\boldsymbol{\mathcal{X}}}
\newcommand{\Ycb}{\boldsymbol{\mathcal{Y}}}
\newcommand{\Zcb}{\boldsymbol{\mathcal{Z}}}


%% Script sets: Capacity region, set of probs, achievable rate region, etc.
\newcommand{\Cr}{\mathscr{C}}
\renewcommand{\Pr}{\mathscr{P}}
\newcommand{\Rr}{\mathscr{R}}
\newcommand{\Ur}{\mathscr{U}}
\newcommand{\Kr}{\mathscr{K}}
\newcommand{\Gr}{\mathscr{G}}
\newcommand{\Sr}{\mathscr{S}}
%% Sequences
%% TODO: Should be cleaned up
\iffalse
\newcommand{\Un}{{U_1,U_2,\ldots,U_n}}
\newcommand{\Vn}{{V_1,V_2,\ldots,V_n}}
\newcommand{\Xk}{{X^{(1)},X^{(2)},\ldots,X^{(k)}}}
\newcommand{\xk}{{x^{(1)},x^{(2)},\ldots,x^{(k)}}}
\newcommand{\Xm}{{X^{(1)},X^{(2)},\ldots,X^{(m)}}}
\newcommand{\xm}{{x^{(1)},x^{(2)},\ldots,x^{(m)}}}
\newcommand{\Xn}{{X_1,X_2,\ldots,X_n}}
\newcommand{\xn}{{x_1,x_2,\ldots,x_n}}
\newcommand{\Ym}{{Y^{(1)},Y^{(2)},\ldots,Y^{(m)}}}
\newcommand{\ym}{{y^{(1)},y^{(2)},\ldots,y^{(m)}}}
\newcommand{\Yn}{{Y_1,Y_2,\ldots,Y_n}}
\newcommand{\yn}{{y_1,y_2,\ldots,y_n}}
\newcommand{\Zn}{{Z_1,Z_2,\ldots,Z_n}}
\newcommand{\zn}{{z_1,z_2,\ldots,z_n}}
\fi


%% Boldface vectors
%%
\newcommand{\av}{\boldsymbol{a}}
\newcommand{\bv}{\boldsymbol{b}}
\newcommand{\cv}{\boldsymbol{c}}
\newcommand{\Lv}{\boldsymbol{L}}
\newcommand{\Xv}{\boldsymbol{X}}
\newcommand{\Yv}{\boldsymbol{Y}}
\newcommand{\Zv}{\boldsymbol{Z}}
\newcommand{\Uv}{\boldsymbol{U}}
\newcommand{\Vv}{\boldsymbol{V}}
\newcommand{\Sv}{\boldsymbol{S}}
\newcommand{\dv}{\boldsymbol{d}}
\newcommand{\fv}{\boldsymbol{f}}
\newcommand{\gv}{\boldsymbol{g}}
\newcommand{\ellv}{\boldsymbol{\ell}}
\newcommand{\lv}{\boldsymbol{l}}
\newcommand{\tv}{\boldsymbol{t}}
\newcommand{\mv}{\boldsymbol{m}}
\newcommand{\xv}{\boldsymbol{x}}
\newcommand{\yv}{\boldsymbol{y}}
\newcommand{\zv}{\boldsymbol{z}}
\newcommand{\uv}{\boldsymbol{u}}
\newcommand{\vv}{\boldsymbol{v}}
\newcommand{\sv}{\boldsymbol{s}}
\newcommand{\rv}{\boldsymbol{r}}
\newcommand{\alphav}{\boldsymbol \alpha}
\newcommand{\betav}{\boldsymbol \beta}
\newcommand{\gammav}{\boldsymbol \gamma}
\newcommand{\muv}{\boldsymbol \mu}
\newcommand{\Deltav}{\boldsymbol \Delta}


%% Typicality
%% \newcommand{\feq}{\stackrel{.}{=}}
\newcommand{\pen}{{P_e^{(n)}}}
\newcommand{\waep}{{\mathcal{A}_{\epsilon}^{(n)}}}
\newcommand{\aep}{{\mathcal{T}_{\epsilon}^{(n)}}}
\newcommand{\aepvar}{{\mathcal{T}_{\epsilon'}^{(n)}}}
\newcommand{\aepvarvar}{{\mathcal{T}_{\epsilon''}^{(n)}}}
\newcommand{\aepb}{{\mathcal{T}_{\epsilon}^{(b)}}}
\newcommand{\aepbvar}{{\mathcal{T}_{\epsilon'}^{(b)}}}
\newcommand{\aepk}{{\mathcal{T}_{\epsilon}^{(k)}}}
%% Typical set with delta in place of epsilon
\newcommand{\aepp}{{\mathcal{T}_{[P]}^{(n)}}}
\newcommand{\aepq}{{\mathcal{T}_{[Q]}^{(n)}}}
\newcommand{\aepw}{{\mathcal{T}_{[W]}^{(n)}}}
\newcommand{\aepv}{{\mathcal{T}_{[V]}^{(n)}}}

%% Hats
\newcommand{\Kh}{{\hat{K}}}
\newcommand{\Lh}{{\hat{L}}}
\newcommand{\Mh}{{\hat{M}}}
\newcommand{\Rh}{{\hat{R}}}
\newcommand{\Sh}{{\hat{S}}}
\newcommand{\Uh}{{\hat{U}}}
\newcommand{\Vh}{{\hat{V}}}
\newcommand{\Wh}{{\hat{W}}}
\newcommand{\Xh}{{\hat{X}}}
\newcommand{\Yh}{{\hat{Y}}}
\newcommand{\Zh}{{\hat{Z}}}
\newcommand{\kh}{{\hat{k}}}
\newcommand{\ellh}{\hat{\ell}}
\newcommand{\lh}{{\hat{l}}}
\newcommand{\mh}{{\hat{m}}}
\newcommand{\sh}{{\hat{s}}}
\newcommand{\uh}{{\hat{u}}}
\newcommand{\vh}{{\hat{v}}}
\newcommand{\wh}{{\hat{w}}}
\newcommand{\xh}{{\hat{x}}}
\newcommand{\yh}{{\hat{y}}}
\newcommand{\zh}{{\hat{z}}}
\newcommand{\gh}{{\hat{g}}}

%% Bars
\newcommand{\Kb}{{\bar{K}}}
\newcommand{\Lb}{{\bar{L}}}
\newcommand{\Mb}{{\bar{M}}}
\newcommand{\Rb}{{\bar{R}}}
\newcommand{\Sb}{{\bar{S}}}
\newcommand{\Ub}{{\bar{U}}}
\newcommand{\Vb}{{\bar{V}}}
\newcommand{\Wb}{{\bar{W}}}
\newcommand{\Xb}{{\bar{X}}}
\newcommand{\Yb}{{\bar{Y}}}
\newcommand{\Zb}{{\bar{Z}}}
\newcommand{\kb}{{\bar{k}}}
\newcommand{\ellb}{\bar{\ell}}
\newcommand{\lb}{{\bar{l}}}
\newcommand{\mb}{{\bar{m}}}
\newcommand{\ub}{{\bar{u}}}
\newcommand{\vb}{{\bar{v}}}
\newcommand{\wb}{{\bar{w}}}
\newcommand{\xb}{{\bar{x}}}
\newcommand{\yb}{{\bar{y}}}
\newcommand{\zb}{{\bar{z}}}
\newcommand{\gb}{{\bar{g}}}


%% Hat Vectors

\newcommand{\Xvh}{\hat{\mathbf{X}}}
\newcommand{\Yvh}{\hat{\mathbf{Y}}}
\newcommand{\Zvh}{\hat{\mathbf{Z}}}
\newcommand{\lvh}{\hat{\mathbf{l}}}
\newcommand{\ellvh}{\hat{\boldsymbol{\ell}}}
\newcommand{\mvh}{\hat{\mathbf{m}}}
\newcommand{\xvh}{\hat{\mathbf{X}}}
\newcommand{\yvh}{\hat{\mathbf{y}}}
\newcommand{\zvh}{\hat{\mathbf{z}}}



%% Tildes
\newcommand{\Kt}{{\tilde{K}}}
\newcommand{\Lt}{{\tilde{L}}}
\newcommand{\Mt}{{\tilde{M}}}
\newcommand{\Rt}{{\tilde{R}}}
\newcommand{\St}{{\tilde{S}}}
\newcommand{\Ut}{{\tilde{U}}}
\newcommand{\Vt}{{\tilde{V}}}
\newcommand{\Wt}{{\tilde{W}}}
\newcommand{\Xt}{{\tilde{X}}}
\newcommand{\Yt}{{\tilde{Y}}}
\newcommand{\Zt}{{\tilde{Z}}}
\newcommand{\dt}{{\tilde{d}}}
\newcommand{\kt}{{\tilde{k}}}
\newcommand{\lt}{{\tilde{l}}}
\newcommand{\mt}{{\tilde{m}}}
\newcommand{\rt}{{\tilde{R}}}
\newcommand{\st}{{\tilde{s}}}
\newcommand{\ut}{{\tilde{u}}}
\newcommand{\vt}{{\tilde{v}}}
\newcommand{\wt}{{\tilde{w}}}
\newcommand{\xt}{{\tilde{x}}}
\newcommand{\yt}{{\tilde{y}}}
\newcommand{\zt}{{\tilde{z}}}
\newcommand{\gt}{{\tilde{g}}}

%% Tilde vectors

\newcommand{\Xvt}{\tilde{\mathbf{X}}}
\newcommand{\Yvt}{\tilde{\mathbf{Y}}}
\newcommand{\Zvt}{\tilde{\mathbf{Z}}}
\newcommand{\xvt}{\tilde{\mathbf{x}}}
\newcommand{\yvt}{\tilde{\mathbf{y}}}
\newcommand{\zvt}{\tilde{\mathbf{z}}}

%% Greek
\def\a{\alpha}
\def\b{\beta}
\def\g{\gamma}
\def\d{\delta}
\def\e{\epsilon}
\def\eps{\epsilon}
\def\l{\lambda}

%% Probability and expectation
\DeclareMathOperator\E{\sf E}
\let\P\relax
\DeclareMathOperator\P{\sf P}
%% \def\E{\mathrm{E}}
%% \def\P{\mathrm{P}}

%% Gaussian capacity, rate-dist, binary entropy
\DeclareMathOperator\C{C}
\DeclareMathOperator\R{R}
\DeclareMathOperator\rr{r}
%%\let\H\relax
%%\DeclareMathOperator\H{H}

%% Error symbol
\def\error{\mathrm{e}}

%% Probability distributions
\newcommand{\Br}{\mathrm{Bern}}
\newcommand{\Bern}{\mathrm{Bern}}
\newcommand{\Geom}{\mathrm{Geom}}
\newcommand{\Poisson}{\mathrm{Poisson}}
\newcommand{\Exp}{\mathrm{Exp}}
\newcommand{\Norm}{\mathrm{N}}
\newcommand{\N}{\mathrm{N}}
\newcommand{\U}{\mathrm{Unif}}
\newcommand{\B}{\mathrm{Binom}}
%% Misc
%%\newcommand\eg{e.g.,\xspace}
%%\newcommand\ie{i.e.,\xspace}
%%\def\textiid{i.i.d.\@\xspace}
%%\newcommand\iid{\ifmmode\text{ i.i.d. } \else \textiid \fi}
%%\let\textand\and
%\renewcommand\and{\ifmmodee{\text{ and }}{\textand}}
%%\let\textor\or
%\renewcommand\or{\ifmmode{\text{ or }}{\textor}}

\newcommand{\geql}{\succeq}
\newcommand{\leql}{\preceq}
\newcommand{\Complex}{\mathbb{C}}
\newcommand{\Real}{\mathbb{R}}
\newcommand{\Integer}{\mathbb{Z}}
\newcommand{\Field}{\mathbb{F}}
\newcommand{\ind}{\boldsymbol{1}}
\newcommand{\defeq}{=}

%% Spacing
\newcommand{\muspace}{\mspace{1mu}}

%% Fractions
\newcommand{\sfrac}[2]{\mbox{\small$\displaystyle\frac{#1}{#2}$}}
\newcommand{\half}{\sfrac{1}{2}}


%Ceiling and Floor
%
%\DeclarePairedDelimiter{\ceil}{\lceil}{\rceil}
%\DeclarePairedDelimiter{\floor}{\lfloor}{\rfloor}

%argmin and argmax
%
%\DeclareMathOperator*{\argmin}{\arg\min}
%\DeclareMathOperator*{\argmax}{\arg\max}


%% For lecture notes
\def\labelitemi{$\bullet$}
\def\labelitemii{$\circ$}


